On the Trap Space Semantics of Normal Logic Programs

The logical semantics of normal logic programs has traditionally been based on the notions of Clark's completion and two-valued or three-valued canonical models, including supported, stable, regular, and well-founded models. Two-valued interpretations can also be seen as states evolving under a program's update operator, producing a transition graph whose fixed points and cycles capture stable and oscillatory behaviors, respectively. We refer to this view as dynamical semantics since it characterizes the program's meaning in terms of state-space trajectories, as first introduced in the stable (supported) class semantics. Recently, we have established a formal connection between Datalog^\neg programs (i.e., normal logic programs without function symbols) and Boolean networks, leading to the introduction of the trap space concept for Datalog^\neg programs. In this paper, we generalize the trap space concept to arbitrary normal logic programs, introducing trap space semantics as a new approach to their interpretation. This new semantics admits both model-theoretic and dynamical characterizations, providing a comprehensive approach to understanding program behavior. We establish the foundational properties of the trap space semantics and systematically relate it to the established model-theoretic semantics, including the stable (supported), stable (supported) partial, regular, and L-stable model semantics, as well as to the dynamical stable (supported) class semantics. Our results demonstrate that the trap space semantics offers a unified and precise framework for proving the existence of supported classes, strict stable (supported) classes, and regular models, in addition to uncovering and formalizing deeper relationships among the existing semantics of normal logic programs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{294}
\providecommand{\publicationstatus}{M. Gebser, D. Inclezan, F. Ricca, M. Carro \& M. Truszczynski:\\
41st International Conference on Logic Programming (ICLP 2025)\\
EPTCS 439, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.439.21}{10.4204/EPTCS.439.21}}


==> main-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndii}Let \(I^*\) be a three-valued interpretation that corresponds to all the two-valued interpretations, i.e., \(\forall a \in \hb {P}, I^*(a) = \star \). By setting \(S = \cset {I^*}\), the condition \(\{\Fop {I} \mid I \in S\} \subseteq S\) (resp.\ \(\{\Top {I} \mid I \in S\} \subseteq S\)) always holds. Hence, \(\cset {I^*}\) is a stable (resp.\ supported) trap set of \(P\). By definition, \(I^*\) is a stable (resp.\ supported) trap space of \(P\).\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndiii}Clearly, \((\stts {P}, \leq _i)\) is a partially ordered set. Consider a \(\leq _i\)-chain \((E_k)_{k \in I}\). Note that \(I\) is the set of all elements of the \(\leq _i\)-chain, and it can be written as an indexed family, which can be done via using the set itself as index set. Consider now the intersection of all elements in \(I\), said \(\sqcap _I\) whose existence is guaranteed by Definition~\ref {def:NLP-intersection-interpretation-consistent-set}. Following from the definition, we have \(\cset {\sqcap _I} = \bigcap _{k \in I}\cset {E_k}\). It follows that \(\sqcap _I \leq _s E_k\) for all \(E_k, k \in I\). Equivalently, \(E_k \leq _i \sqcap _I\) for all \(E_k, k \in I\), implying that \(\sqcap _I\) is an upper bound w.r.t. \(\leq _i\) of \((E_k)_{k \in I}\). It remains to show that \(\sqcap _I\) is a stable trap space of \(P\). \par Consider a two-valued interpretation \(A\) of \(P\). Let \(B\) be the successor of \(A\) in \(\tgst {P}\), i.e., \(B = \Fop {A}\). Assume that \(A \in \cset {\sqcap _I}\). Then for all \(k \in I\), we have that \(A \in \cset {E_k}\). Thus \(B \in \cset {E_k}\), since \(E_k\) is a stable trap space. Hence, \(B \in \cset {\sqcap _I}\). This implies that if \(A \in \cset {\sqcap _I}\) then \(\Fop {A} \in \cset {\sqcap _I}\), thus \(\sqcap _I\) is a stable trap set of \(P\). Since \(\sqcap _I\) is a three-valued interpretation by definition, it is a stable trap space of \(P\). \par By definition, a \(\leq _s\)-minimal stable trap space is equivalent to a \(\leq _i\)-maximal stable trap space. By Lemma~\ref {lem:Zorn-lemma-strengthened}, if \(J\) is a stable trap space of \(P\), then there exists a \(\leq _s\)-minimal stable trap space \(J'\) of \(P\) such that \(J \leq _i J'\) (equivalently, \(J' \leq _s J\)).\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndiv}The proof of Lemma~\ref {lem:NLP-SuTS-min-s-SuTS} can be applied here by substituting \(\Fop {A}\) in Lemma~\ref {lem:NLP-StTS-min-s-StTS} with \(\Top {A}\).\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndv}For the case of \(\leq _s\)-minimal stable trap spaces, this immediately follows from Lemma~\ref {lem:NLP-StTS-min-s-StTS} and the fact that \(P\) has at least one stable trap space by Proposition~\ref {prop:NLP-exist-St-Su-TS}. \par For the case of \(\leq _s\)-minimal supported trap spaces, this immediately follows from Lemma~\ref {lem:NLP-SuTS-min-s-SuTS} and the fact that \(P\) has at least one supported trap space by Proposition~\ref {prop:NLP-exist-St-Su-TS}.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndvi}Hereafter, we prove the case of stable trap spaces. The proof for the case of supported trap spaces is analogous. Let \(T\) be the set of all stable trap spaces \(I\) such that \(S \subseteq \cset {I}\). The set \(T\) is non-empty as it contains \(\epsilon \) that is a stable trap space in which all atoms are assigned to \(\uval \) (see Proposition~\ref {prop:NLP-exist-St-Su-TS}). Since \(S\) is non-empty, the elements in \(T\) are mutually consistent, thus we can take the intersection of all these elements said \(\sqcap _T\). \par Next, we show that \(\sqcap _T\) is also a stable trap space of \(P\). Consider a two-valued interpretation \(A\) of \(P\). Let \(B\) be the successor of \(A\) in \(\tgst {P}\), i.e., \(B = \Fop {A}\). Assume that \(A \in \cset {\sqcap _T}\). Then for all \(E_k \in T\), we have that \(A \in \cset {E_k}\). Thus \(B \in \cset {E_k}\), since \(E_k\) is a stable trap space. Hence, \(B \in \cset {\sqcap _T}\). This implies that if \(A \in \cset {\sqcap _T}\) then \(\Fop {A} \in \cset {\sqcap _T}\), thus \(\sqcap _T\) is a stable trap set of \(P\). Since \(\sqcap _T\) is a three-valued interpretation by definition, it is a stable trap space of \(P\). \par By definition, \(\sqcap _T\) is unique and \(\leq _s\)-minimal. Since \(S \subseteq \cset {E_k}\) for all \(E_k \in T\), \(S \subseteq \cset {\sqcap _T}\). By setting \(\langle S\rangle ^{st}_{P} = \sqcap _T\), we can conclude the proof.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndvii}Hereafter, we prove the case of stable trap spaces. The proof for the case of supported trap spaces is analogous. Assume that \(I_1\) and \(I_2\) are consistent. Then \(I = \sqcap _{\{I_1, I_2\}}\) exists and \(\cset {I} = \cset {I_1} \cap \cset {I_2}\). By similarly applying the arguments of Proposition~\ref {prop:NLP-unique-minimal-covered-TS}, we have \(I\) is also a stable trap space of \(P\). Since \(I_1\) and \(I_2\) are distinct, we have \(\cset {I_1} \subset \cset {I}\) or \(\cset {I_2} \subset \cset {I}\) must hold. This leads to a contradiction because \(I_1\) and \(I_2\) are \(\leq _s\)-minimal stable trap spaces of \(P\). Hence, \(I_1\) and \(I_2\) are not consistent.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndviii}Let \(TS(P)\) denote the set of all stable trap sets of \(P\). Clearly, \((TS(P), \supseteq )\) is a partially ordered set. Given a \(\supseteq \)-chain \((E_i)_{i \in I}\). Note that \(I\) is the set of all elements of the \(\supseteq \)-chain, and it can be written as an indexed family, which can be done via using the set itself as index set. Consider now \(E = \bigcap _{i \in I}E_i\). Obviously, \(E\) is an upper bound of \((E_i)_{i \in I}\), i.e., \(E_i \supseteq E\), for all \(i \in I\). It remains to show that \(E\) is a stable trap set of \(P\). \par Consider a two-valued interpretation \(A\). \(A \in E\) \ifftext \(A \in E_i, \forall i \in I\). This implies that \(\Fop {A} \in E_i, \forall i \in I\) since \(E_i\) is a stable trap set of \(P\). Then \(\Fop {A} \in E\). This implies that \(\{\Fop {B} \mid B \in E\} \subseteq E\). By definition, \(E\) is a stable trap set of \(P\). \par By definition, \(\subseteq \)-minimal stable trap set is equivalent to a \(\supseteq \)-maximal stable trap set. By Lemma~\ref {lem:Zorn-lemma-strengthened}, if \(S\) is a stable trap set of \(P\), then there exists a \(\subseteq \)-minimal stable trap set \(S'\) of \(P\) such that \(S \supseteq S'\) (equivalently, \(S' \subseteq S\)).\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndix}The proof of Lemma~\ref {lem:NLP-St-trap-set-min-s} can be applied here by substituting \(\Fop {I}\) in Lemma~\ref {lem:NLP-St-trap-set-min-s} with \(\Top {I}\).\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndx}``\(\Rightarrow \)'' Assume that \(S\) is a \(\subseteq \)-minimal stable trap set of \(P\). Then \(\{\Fop {I} \mid I \in S\} \subseteq S\) by definition. Suppose that \(\{\Fop {I} \mid I \in S\} \subsetneq S\). Then there exists \(J \in S\) such that for all \(I \in S\), \(\Fop {I} \neq J\). We have \(\{\Fop {I} \mid I \in S \setminus \{J\}\} \subseteq \{\Fop {I} \mid I \in S\} \subseteq S \setminus \{J\}\). Thus \(S \setminus \{J\}\) is a stable trap set of \(P\), which contradicts the \(\subseteq \)-minimality of \(S\). Hence \(\{\Fop {I} \mid I \in S\} = S\), i.e., \(S\) is a stable class of \(P\). Since a stable class is a stable trap set, \(S\) must be a strict stable class. \par ``\(\Leftarrow \)'' Assume that \(S\) is a strict stable class of \(P\). Then \(\{\Fop {I} \mid I \in S\} = S\) by definition. This implies that \(S\) is a stable trap set of \(P\). By Lemma~\ref {lem:NLP-St-trap-set-min-s}, there is a \(\subseteq \)-minimal stable trap set \(S'\) such that \(S' \subseteq S\). We have \(\{\Fop {I} \mid I \in S'\} \subseteq S'\) by definition. Suppose that \(\{\Fop {I} \mid I \in S'\} \subsetneq S'\). Then there is \(J \in S'\) such that \(\Fop {I} \neq J\) for all \(I \in S'\). We have \(\{\Fop {I} \mid I \in S' \setminus \{J\}\} \subseteq \{\Fop {I} \mid I \in S'\} \subseteq S' \setminus \{J\}\). By definition, \(S' \setminus \{J\}\) is a stable trap set of \(P\), which contradicts the \(\subseteq \)-minimality of \(S'\). Thus, \(\{\Fop {I} \mid I \in S'\} = S'\), i.e., \(S'\) is a stable class of \(P\). \(S\) is a strict stable class of \(P\), thus \(S = S'\) because of the \(\subseteq \)-minimality of a strict stable class. Hence, \(S\) is a \(\subseteq \)-minimal stable trap set of \(P\).\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxi}The proof of Theorem~\ref {theo:NLP-min-St-trap-set-strict-StC} can be applied here by substituting \(\Fop {I}\) and Lemma~\ref {lem:NLP-St-trap-set-min-s} in Theorem~\ref {theo:NLP-min-St-trap-set-strict-StC} with \(\Top {I}\) and Lemma~\ref {lem:NLP-Su-trap-set-min-s}, respectively.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxii}Assume that \(I\) is a stable trap space of \(P\). By definition, \(\cset {I}\) is a stable trap set of \(P\). There exists a \(\subseteq \)-minimal stable trap set \(S' \subseteq \cset {I}\). By Theorem~\ref {theo:NLP-min-St-trap-set-strict-StC}, \(S'\) is also a strict stable class of \(P\). \par Assume that \(I\) is a supported trap space of \(P\). By definition, \(\cset {I}\) is a supported trap set of \(P\). There exists a \(\subseteq \)-minimal supported trap set \(S' \subseteq \cset {I}\). By Theorem~\ref {theo:NLP-min-Su-trap-set-strict-SuC}, \(S'\) is also a strict supported class of \(P\).\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxiii}We prove the case of strict stable classes first. \par Let \(S_1\) and \(S_2\) be two distinct strict stable classes of \(P\). By Theorem~\ref {theo:NLP-min-St-trap-set-strict-StC}, \(S_1\) and \(S_2\) are two distinct \(\subseteq \)-minimal stable trap sets of \(P\). Assume that \(S_1\) and \(S_2\) are not disjoint. It follows that \(S_1 \cap S_2 \neq \emptyset \). Consider \(I \in S_1 \cap S_2\). We have \(I \in S_1\) and \(I \in S_2\), then \(\Fop {I} \in S_1\) and \(\Fop {I} \in S_2\) because \(S_1\) and \(S_2\) are stable trap sets, thus \(\Fop {I} \in S_1 \cap S_2\). It follows that \(S_1 \cap S_2\) is a stable trap set of \(P\). Then \(S_1 \cap S_2 \subsetneq S_1\) or \(S_1 \cap S_2 \subsetneq S_2\) must hold because \(S_1 \neq S_2\), which contradicts the \(\subseteq \)-minimality of \(S_1\) and \(S_2\). Hence, \(S_1\) and \(S_2\) are disjoint. \par For the case of strict supported classes, we only need to replace \(F_P\) and Theorem~\ref {theo:NLP-min-St-trap-set-strict-StC} with \(T_P\) and Theorem~\ref {theo:NLP-min-Su-trap-set-strict-SuC}, respectively.\end{proof}

\prAtEndRestatexiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxiv}``\(\Rightarrow \)'' Assume that \(I\) is a supported trap space of \(P\). Suppose that there is an atom \(a \in \hb {P}\) such that \(I(a) <_s I(\rhs {a})\). By the definition of the order \(\leq _s\), we have \(I(\rhs {a}) = \uval \) and \(I(a) \neq \uval \). Since \(I(\rhs {a}) = \uval \), there exists a two-valued interpretation \(J \in \cset {I}\) such that \(J(\rhs {a}) = \neg I(a)\). By definition, \(\Top {J}(a) = J(\rhs {a})\), thus \(\Top {J}\) does not belong to \(\cset {I}\). This implies that \(\cset {I}\) is not a supported trap set by definition, which is a contradiction. Hence, \(I(\rhs {a}) \leq _s I(a)\) for every \(a \in \hb {P}\). \par ``\(\Leftarrow \)'' Assume that \(I(\rhs {a}) \leq _s I(a)\) for every atom \(a \in \hb {P}\). Let \(A\) be a two-valued interpretation in \(\cset {I}\). Of course, \(A \leq _s I\). By the characteristics of the three-valued logic, we have \(A(\rhs {a}) \leq _s I(\rhs {a})\), then \(A(\rhs {a}) \leq _s I(a)\) for every \(a \in \hb {P}\). This implies that \(\Top {A} \leq _s I\), thus \(\Top {A} \in \cset {I}\). Hence, \(\cset {I}\) is a supported trap set of \(P\). By definition, \(I\) is a supported trap space of \(P\).\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxv}It has been shown in~\cite {IS2012} that for any two-valued interpretation \(I\), \(\Fop {I} = \Top {I}\), if \(P\) is a negative \nlp . By the definitions of stable and supported transition graphs, we have that \(\tgst {P} = \tgsp {P}\).\end{proof}

\prAtEndRestatexvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxvi}This immediately follows from Theorem~\ref {theo:neg-NLP-StTG-SuTG}.\end{proof}

\prAtEndRestatexvii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxvii}It has been shown in~\cite {IS2012} that for any two-valued interpretation \(I\), we have that \(\Fop {I} = F_{\lfp {P}}(I)\). By the definition of stable transition graph, we have that \(\tgst {P} = \tgst {\lfp {P}}\).\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxviii}This immediately follows from Theorem~\ref {theo:NLP-lfp-StTG}.\end{proof}

\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxix}Assume that \(I\) is a supported partial model of \(P\). Then \(I\) is a three-valued model of \(\comp {P}\). It follows that \(I(a) = I(\rhs {a})\), \(\forall a \in \hb {P}\). Thus, \(I\) also satisfies the condition \(I(\rhs {a}) \leq _s I(a)\), \(\forall a \in \hb {P}\). By Theorem~\ref {theo:NLP-char-SuTS}, \(I\) is also a supported trap space of \(P\).\end{proof}

\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxx}Assume that \(I\) is a stable partial model of \(P\). \\ Then \(I\) is also a stable partial model of \(\lfp {P}\) by Theorem~\ref {theo:NLP-lfp-model-equivalence}. \\ Since \(\lfp {P}\) is a negative \nlp , \(I\) is also a supported partial model of \(\lfp {P}\) by Theorem~\ref {theo:neg-NLP-StPM-SuPM}. \\ By Proposition~\ref {prop:NLP-SuPM-is-SuTS}, \(I\) is a supported trap space of \(\lfp {P}\). \\ By Corollary~\ref {cor:neg-NLP-StTS-SuTS}, \(I\) is also a stable trap space of \(\lfp {P}\). \\ By Corollary~\ref {cor:NLP-lfp-StTS}, \(I\) is a stable trap space of \(P\).\end{proof}

\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxi}By definition, \(f_P(I)(v) = I(\rhs {v})\) for all \(v \in \hb {P}\). Since \(I\) is a supported trap space of \(P\), \(I(v) \leq _i I(\rhs {v})\) for all \(v \in \hb {P}\) by Theorem~\ref {theo:NLP-char-SuTS}. Thus, \(I \leq _i f_P(I)\). Then, by the truth table of the three-valued logic, \(I(\rhs {v}) \leq _i f_P(I)(\rhs {v})\) for all \(v \in \hb {P}\). This implies that \(f_P(I)(v) \leq _i f_P(I)(\rhs {v})\) for all \(v \in \hb {P}\). Hence, \(f_P(I)\) is a supported trap space of \(P\) by Theorem~\ref {theo:NLP-char-SuTS}.\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxii}We define a function \(K\) recursively on the ordinals as follows: \begin {align*} K(0) &= I \\ K(\alpha + 1) &= f_P(K(\alpha )). \end {align*} If \(\beta \) is a limit ordinal, then by construction and Lemma~\ref {lem:NLP-next-SuTS} \(\{K(\alpha ) \colon \alpha < \beta \}\) is a chain w.r.t. \(\leq _i\) in \(\suts {P}\). Define \(K(\beta ) = \text {sup}_{\leq _i}\{K(\alpha ) \colon \alpha < \beta \}\), where \(\text {sup}_{\leq _i}\) denotes the least upper bound w.r.t. \(\leq _i\). We have \(K\) is an increasing function from the ordinals into \(\suts {P}\). It cannot be strictly increasing, as if it was, then we would have an injection from the ordinals into \(\suts {P}\), which violates Lemma~\ref {lem:Hartogs}. Hence, \(K\) must be eventually constant. It follows that for some ordinal \(\alpha \), \(K(\alpha + 1) = K(\alpha )\), then \(f_P(K(\alpha )) = K(\alpha )\). Let \(\alpha ^*\) be the least ordinal such that \(K(\alpha ^* + 1) = K(\alpha ^*)\). We have \(K(\beta ) = K(\alpha ^*)\) for all \(\beta > \alpha ^*\). Hence, \(K(\alpha ^*)\) is unique. Set \(I' = K(\alpha ^*)\). We have \(f_P(I') = I'\), i.e., \(I'\) is a three-valued model of \(\comp {P}\). Therefore, \(I' \in \supms {P}\). By construction and Lemma~\ref {lem:NLP-next-SuTS}, \(I \leq _i I'\). This implies that \(I' \leq _s I\).\end{proof}

\prAtEndRestatexxiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxiii}Recall that \(\suts {P}\) (resp.\ \(\supms {P}\)) denotes the set of all supported trap spaces (resp.\ partial models) of \(P\). We have \(\supms {P} \subseteq \suts {P}\) by Proposition~\ref {prop:NLP-SuPM-is-SuTS}. \par ``\(\Rightarrow \)'' Assume that \(I\) is not a \(\leq _s\)-minimal supported trap space of \(P\). Then there exists \(I' \in \suts {P}\) such that \(I' <_s I\). By Theorem~\ref {theo:NLP-SuTS-reach-unique-SuPM}, there exists \(J \in \supms {P}\) such that \(J \leq _s I'\). This implies that \(J <_s I\), which contradicts the \(\leq _s\)-minimality of \(I\). Hence, \(I\) is a \(\leq _s\)-minimal supported trap space of \(P\). \par ``\(\Leftarrow \)'' This direction is trivial because \(\supms {P} \subseteq \suts {P}\).\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxiv}Consider \(J \in S\). Since \(S \subseteq \cset {I}\), we have \(J \in \cset {I}\). Let \(J' = \Top {J}\). For any atom \(a \in \hb {P}\), we have \(J'(a) = J(\rhs {a}) \leq _s I(\rhs {a}) = f_{P}(I)(a)\). This implies that \(J' \in \cset {f_{P}(I)}\). Hence, \(\{\Top {J} \mid J \in S\} \subseteq \cset {f_{P}(I)}\). Since \(S\) is a supported class, \(\{\Top {J} \mid J \in S\} = S\) by definition. This implies that \(S \subseteq \cset {f_{P}(I)}\).\end{proof}

\prAtEndRestatexxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxv}By Proposition~\ref {prop:NLP-unique-minimal-covered-TS}, \(\langle S\rangle ^{sp}_{P}\) is a supported trap space of \(P\). Assume that it is not a supported partial model of \(P\). Then by definition, we have \(f_{P}(\langle S\rangle ^{sp}_{P}) \neq \langle S\rangle ^{sp}_{P}\). By Lemma~\ref {lem:NLP-next-SuTS}, \(f_{P}(\langle S\rangle ^{sp}_{P}) \leq _s \langle S\rangle ^{sp}_{P}\). It follows that \(f_{P}(\langle S\rangle ^{sp}_{P}) <_s \langle S\rangle ^{sp}_{P}\). By Lemma~\ref {lem:NLP-SuC-in-next-interpretation}, \(S \subseteq \cset {f_{P}(\langle S\rangle ^{sp}_{P})}\) because \(S\) is a supported class and \(S \subseteq \cset {\langle S\rangle ^{sp}_{P}}\) by definition. This implies that \(\langle S\rangle ^{sp}_{P}\) is not a \(\leq _s\)-minimal supported trap space covering \(S\), which is a contradiction. Hence, \(\langle S\rangle ^{sp}_{P}\) is a supported partial model of \(P\).\end{proof}

\prAtEndRestatexxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxvi}By Theorem~\ref {theo:NLP-lfp-StTG} and Theorem~\ref {theo:neg-NLP-StTG-SuTG}, \(\tgst {P} = \tgst {\lfp {P}} = \tgsp {\lfp {P}}\). Hence, \(S\) is a supported class of \(\lfp {P}\). In addition, \(\langle S\rangle ^{st}_{P} = \langle S\rangle ^{sp}_{\lfp {P}}\). By Proposition~\ref {prop:NLP-SuPM-cover-SuC}, \(\langle S\rangle ^{sp}_{\lfp {P}}\) is a supported partial model of \(\lfp {P}\). It is also a stable partial model of \(\lfp {P}\) by Theorem~\ref {theo:neg-NLP-StPM-SuPM}, since \(\lfp {P}\) is negative. By Theorem~\ref {theo:NLP-lfp-model-equivalence}, \(\langle S\rangle ^{st}_{P}\) is a stable partial model of \(P\).\end{proof}

\prAtEndRestatexxvii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxvii}The programs \(P\) and \(\lfp {P}\) have the same set of regular models by Theorem~\ref {theo:NLP-lfp-model-equivalence}. They also have the same set of stable trap spaces by Corollary~\ref {cor:NLP-lfp-StTS}. Hence, it suffices to show that \(I\) is a regular model of \(\lfp {P}\) \ifftext \(I\) is a \(\leq _s\)-minimal stable trap space of \(\lfp {P}\). \par Recall that \(\lfp {P}\) is a negative NLP. Then \(I\) is a regular model of \(\lfp {P}\) \\ \ifftext \(I\) is a \(\leq _s\)-minimal stable partial model of \(\lfp {P}\) by definition \\ \ifftext \(I\) is a \(\leq _s\)-minimal supported partial model of \(\lfp {P}\) by Theorem~\ref {theo:neg-NLP-StPM-SuPM} \\ \ifftext \(I\) is a \(\leq _s\)-minimal supported trap space of \(\lfp {P}\) by Corollary~\ref {cor:NLP-min-s-SuPM-min-s-SuTS} \\ \ifftext \(I\) is a \(\leq _s\)-minimal stable trap space of \(\lfp {P}\) by Corollary~\ref {cor:neg-NLP-StTS-SuTS}.\end{proof}

\prAtEndRestatexxviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxviii}We have \(I_1 \leq _u I_2\) \\ \ifftext \(I_1(v) \leq _u I_2(v)\) for all \(v \in \hb {P}\) \\ \ifftext either \(I_1(v), I_2(v) \neq \star \) or \(I_1(v) <_u I_2(v)\) for all \(v \in \hb {P}\) \\ \ifftext \(I_1^{\textbf {u}} \subseteq I_2^{\textbf {u}}\).\end{proof}

\prAtEndRestatexxix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxix}This immediately follows from Proposition~\ref {prop:NLP-u-order-subset}.\end{proof}

\prAtEndRestatexxx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxx}By Theorem~\ref {theo:NLP-SuTS-reach-unique-SuPM}, there is a unique supported partial model \(J \in \supms {P}\) such that \(J \leq _s I\). Since \(I' \leq _s I\) implies \(I' \leq _u I\), we can conclude the proof. Note that for \(\leq _u\), such a supported partial model may not be unique.\end{proof}

\prAtEndRestatexxxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxi}We have \(\supms {P} \subseteq \suts {P}\) by Proposition~\ref {prop:NLP-SuPM-is-SuTS}. \par ``\(\Rightarrow \)'' Assume that \(I\) is not a \(\leq _u\)-minimal supported trap space of \(P\). Then there exists \(I' \in \suts {P}\) such that \(I' <_u I\). By Proposition~\ref {prop:NLP-SuTS-reach-u-SuPM}, there exists \(J \in \supms {P}\) such that \(J \leq _u I'\). This implies that \(J <_u I\), which contradicts the \(\leq _u\)-minimality of \(I\). Hence, \(I\) is a \(\leq _u\)-minimal supported trap space of \(P\). \par ``\(\Leftarrow \)'' This direction is trivial because \(\supms {P} \subseteq \suts {P}\).\end{proof}

\prAtEndRestatexxxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxii}We have \(P\) and \(\lfp {P}\) have the same set of stable partial models by Theorem~\ref {theo:NLP-lfp-model-equivalence}. They also have the same set of stable trap spaces by Corollary~\ref {cor:NLP-lfp-StTS}. Hence, it suffices to show that \(I\) is an L-stable model of \(\lfp {P}\) \ifftext \(I\) is a \(\leq _u\)-minimal stable trap space of \(\lfp {P}\). \par Recall that \(\lfp {P}\) is a negative NLP. We have \(I\) is an L-stable model of \(\lfp {P}\) \\ \ifftext \(I\) is a \(\leq _u\)-minimal stable partial model of \(\lfp {P}\) by Corollary~\ref {cor:NLP-L-StM-u-min-StPM} \\ \ifftext \(I\) is a \(\leq _u\)-minimal supported partial model of \(\lfp {P}\) by Theorem~\ref {theo:neg-NLP-StPM-SuPM} \\ \ifftext \(I\) is a \(\leq _u\) supported trap space of \(\lfp {P}\) by Corollary~\ref {cor:NLP-u-min-SuPM-u-min-SuTS} \\ \ifftext \(I\) is a \(\leq _u\)-minimal stable trap space of \(\lfp {P}\) by Corollary~\ref {cor:neg-NLP-StTS-SuTS}.\end{proof}

\prAtEndRestatexxxiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxiii}By Theorem~\ref {theo:NLP-L-StM-u-min-StTS}, it suffices to show that \(I\) is a \(\leq _u\)-minimal stable trap space of \(P\) \ifftext \(I\) is a \(\leq _u\)-minimal regular model of \(P\). The forward direction is trivial because \(\regms {P} \subseteq \stts {P}\), i.e., the set of regular models is a subset of the set of stable trap spaces. Now, we prove the backward direction. \par Assume that \(I\) is a \(\leq _u\)-minimal regular model of \(P\). Then \(I\) is a \(\leq _u\)-minimal regular model of \(\lfp {P}\) by Theorem~\ref {theo:NLP-lfp-model-equivalence}. Suppose that \(I\) is not a \(\leq _u\)-minimal stable trap space of \(\lfp {P}\). Then there is a stable trap space \(I'\) of \(\lfp {P}\) such that \(I' <_u I\). By Theorem~\ref {theo:NLP-RegM-s-min-StTS}, the regular models of \(\lfp {P}\) are the \(\leq _s\)-minimal stable trap spaces of \(\lfp {P}\). This implies that there is a regular model \(J\) of \(\lfp {P}\) such that \(J \leq _s I'\). Since \(J \leq _s I'\) implies \(J \leq _u I'\), \(J <_u I\). By Theorem~\ref {theo:NLP-lfp-model-equivalence}, \(J\) is a regular model of \(P\), which contradicts the \(\leq _u\)-minimality of \(I\). Hence, \(I\) is a \(\leq _u\)-minimal stable trap space of \(\lfp {P}\). By Corollary~\ref {cor:NLP-lfp-StTS}, \(I\) is a \(\leq _u\)-minimal stable trap space of \(P\).\end{proof}

\prAtEndRestatexxxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxiv}By Proposition~\ref {prop:NLP-L-StM-u-min-RegM}, the set of L-stable models of \(P\) coincides with the set of \(\leq _u\)-minimal regular models of \(P\). If \(\regms {P}\) is a finite set, then it always has a \(\leq _u\)-minimal element, i.e., the set of \(\leq _u\)-minimal regular models of \(P\) is non-empty, leading to \(P\) has an L-stable model, which is a contradiction. Hence, \(P\) has infinitely many regular models.\end{proof}

\prAtEndRestatexxxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxv}For the case of \(\subseteq \)-minimal stable trap sets, this immediately follows from Lemma~\ref {lem:NLP-St-trap-set-min-s} and the fact that \(P\) has at least one stable trap set by Proposition~\ref {prop:NLP-exist-St-Su-TS}. \par For the case of \(\subseteq \)-minimal supported trap sets, this immediately follows from Lemma~\ref {lem:NLP-Su-trap-set-min-s} and the fact that \(P\) has at least one supported trap set by Proposition~\ref {prop:NLP-exist-St-Su-TS}.\end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Alternative proof of Theorem 5.1]\phantomsection\label{proof:prAtEndxxxv}By Theorem~\ref {theo:NLP-exist-min-trap-set}, \(P\) has a \(\subseteq \)-minimal stable trap set \(S\). We show that \(S\) is a stable class. \par By definition, \(\{\Fop {I} \mid I \in S\} \subseteq S\). Suppose that \(\{\Fop {I} \mid I \in S\} \subsetneq S\). Then there exists \(J \in S\) such that for all \(I \in S\), \(\Fop {I} \neq J\). We have \(\{\Fop {I} \mid I \in S \setminus \{J\}\} \subseteq \{\Fop {I} \mid I \in S\} \subseteq S \setminus \{J\}\). Thus \(S \setminus \{J\}\) is a supported trap set of \(P\), which contradicts the \(\subseteq \)-minimality of \(S\). Hence \(\{\Fop {I} \mid I \in S\} = S\), i.e., \(S\) is a supported class of \(P\).\end{proof}

\prAtEndRestatexxxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxvi}By Theorem~\ref {theo:NLP-exist-min-trap-set}, \(P\) has a \(\subseteq \)-minimal supported trap set \(S\). We show that \(S\) is a supported class. \par By definition, \(\{\Top {I} \mid I \in S\} \subseteq S\). Suppose that \(\{\Top {I} \mid I \in S\} \subsetneq S\). Then there exists \(J \in S\) such that for all \(I \in S\), \(\Top {I} \neq J\). We have \(\{\Top {I} \mid I \in S \setminus \{J\}\} \subseteq \{\Top {I} \mid I \in S\} \subseteq S \setminus \{J\}\). Thus \(S \setminus \{J\}\) is a supported trap set of \(P\), which contradicts the \(\subseteq \)-minimality of \(S\). Hence \(\{\Top {I} \mid I \in S\} = S\), i.e., \(S\) is a supported class of \(P\).\end{proof}

\prAtEndRestatexxxvii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxvii}This immediately follows from Theorem~\ref {theo:NLP-exist-min-trap-set} and Theorem~\ref {theo:NLP-min-St-trap-set-strict-StC} (resp.\ Theorem~\ref {theo:NLP-min-Su-trap-set-strict-SuC}).\end{proof}

\prAtEndRestatexxxviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndxxxviii}This immediately follows from Theorem~\ref {theo:NLP-RegM-s-min-StTS} and Theorem~\ref {theo:NLP-exist-min-s-StTS-SuTS}.\end{proof}

